Simulating Performance of a BitTorrent-Based P2P TV System

In this paper we describe a prototype of a simulation framework and some ideas which are to be used to study performance of a P2P TV system in a controllable and adjustable environment. We created a simplified model describing live video distribution in a P2P TV system. Using the model we analyse how some of the system parameters influence its behaviour. We present the preliminary results obtained at different granularity levels of measurements, describing the macroscopic system performance as well as the performance of its individual components.

==> fig/pscol <==
#!/usr/bin/perl

#=======================================================================
# pscol: changes RGB color to GRAY or CMYK
#-----------------------------------------------------------------------
# Programmer: Patrick Joeckel (joeckel@mpch-mainz.mpg.de)
#             Max Planck Institute for Chemistry
# Version: 0.1b
# Date: 03 Apr 2002
#
# The program works with AFPL Ghostscript output (e.g., ps2ps, eps2eps)
#
#    This program is a heavily modified and simplified version
#    of 'psmod' (Niklas Nordin, Chalmers University of Technology,
#                09 Sep 2000, v1.0.2,
#                http://www.tfd.chalmers.se/~nordin/psmod/ )
#
# ...You may distribute this program freely...
#=======================================================================

use strict;
use English;
use FileHandle;

#=======================================================================
# global variables
#=======================================================================
my $version = "0.1b";
my $numargs = scalar @ARGV;
my $infilename,my $outfilename;
my $red, my $green, my $blue;
my $K, my $C, my $M, my $Y;
my $gray ;
my $colorline = 0;
my $epsHeader      = "%!PS-Adobe-3.0 EPSF-3.0\n";

my $low = 0.001;
my $high = 0.999;
my $delta = ($high - $low)/4.0;
#=======================================================================
# flags
#=======================================================================
# -h
my $help = 0;

# -gray
my $toGray = 0;

# -0gray
my $to0Gray = 0;

# -cmyk
# using the formula below
# K = min( 1 - $red, 1 - $green, 1 - $blue )
# C = ( 1 - $red - K ) / ( 1 - K )
# M = ( 1 - $green - K ) / ( 1 - K )
# Y = ( 1 - $blue - K ) / ( 1 - K )
my $toCMYK = 0;
#=======================================================================

#=======================================================================
# MAIN
#=======================================================================
if ($numargs eq 0 ) {
   &printHelp ;
   exit(0);
} 

# Check flags and get filename
foreach $a (@ARGV) {
  if (substr($a, 0, 1) eq "-") {
	if ( ( $a eq "-h" )|| ( $a eq "-help" ) || ( $a eq "--help" ) ) {
	    &printHelp;
	    exit(0);
	}
	elsif ( $a eq "-gray" ) {
	  $toGray = 1;
	}
	elsif ( $a eq "-0gray" ) {
	  $to0Gray = 1;
	}
	elsif ( $a eq "-cmyk" ) {
	  $toCMYK = 1;
	}
	else {
	  &unknownFlag;
	  exit(0);
	}
  }
}

if ($numargs eq 3 ) {
    $infilename = $ARGV[1];
    $outfilename = $ARGV[2];
} else {
    &printHelp;
    exit(1);
}


if (! -e $infilename) {
    print "File $infilename does not exist. Exit !\n";
    exit(0);
}

if (-e $outfilename) {
    print "File $outfilename exists. Exit !\n";
    exit(1);
}

print "\nParsing '$infilename' ... ";

open(READ, $infilename) or die "Can't open `$infilename': $!\n";
open (DATA, ">" . $outfilename);

while(<READ>) {
    my $tmpLine = $_;
    ### RESET
    $colorline = 0;

    ### SOME HEADER INFORMATION
    if (/%%EndComments/) {
	print DATA "%%Modified by pscol v$version (";
	print DATA localtime() . ")\n";
	if ($toCMYK) {
	    print DATA "/Ck{setcmykcolor} def %%pscol v$version\n";
	}
    }

    ### GET COLOR
    # rG 
    if (/\d* \d* \d* rG/) {
	$colorline = 1;
	split;
	$red = $_[0]/255;
	$green = $_[1]/255;
	$blue = $_[2]/255;
    }
    # r3
    if (/\d* \d* r3/) {
	$colorline = 2;
	split;
	$red = $_[0]/255;
	$green = $_[1]/255;
	$blue = $_[1]/255;
    }
    # r5
    if (/\d* \d* r5/) {
	$colorline = 3;
	split;
	$red = $_[1]/255;
	$green = $_[0]/255;
	$blue = $_[1]/255;
    }
    # r6
    if (/\d* \d* r6/) {
	$colorline = 4;
	split;
	$red = $_[1]/255;
	$green = $_[1]/255;
	$blue = $_[0]/255;
    }

    if ( $colorline gt 0) {
	### CONVERT COLOR ...
	### ... to GRAY
	if ( $toGray ) {
	    &calculateGray;
	    $gray = $gray*255;
	    print DATA "$gray G\n";
	}
	if ( $to0Gray ) {
	    &calculate0Gray;
	    $gray = $gray*255;
	    print DATA "$gray G\n";
	}
	### ... to CMYK
	if ( $toCMYK ) {
	    &calculateCMYK;	    
	    $C = $C;
	    $M = $M;
	    $Y = $Y;
	    $K = $K;
	    print DATA sprintf("%6.4f %6.4f %6.4f %6.4f Ck\n",,$C,$M,$Y,$K);
	}
    } else {
	### KEEP LINE AS IS
	print DATA $tmpLine;
    }
}

close (DATA);
close (READ);
print "\nCreated '$outfilename'.\n";
print "Done !\n\n";
#
#=======================================================================

#=======================================================================
#  subroutine calculateCMYK
#=======================================================================
sub calculateCMYK {

  $C = 0.0;
  $M = 0.0;
  $Y = 0.0;
  
  if ( 1.0 - $red < 1.0 - $green ) { $K = 1.0 - $red }
  else { $K = 1.0 - $green }
  if ( 1.0 - $blue < $K ) { $K = 1.0 -$blue }
  if ( $K != 1.0 ) {
	$C = ( 1.0 - $red - $K ) / ( 1.0 - $K );
	$M = ( 1.0 - $green - $K ) / ( 1.0 - $K );
	$Y = ( 1.0 - $blue - $K ) / ( 1.0 - $K );
  } 

}
#=======================================================================

#=======================================================================
#  subroutine calculate0Gray
#=======================================================================
sub calculate0Gray {

  my $sum = $red + $green + $blue;
  $gray = $sum/3.0;
}
#=======================================================================

#=======================================================================
#  subroutine calculateGray
#=======================================================================
sub calculateGray {

  my $sum = $red + $green + $blue;

  if ( ($sum != 0.0) && ($sum != 3.0)) {
	if ( $red == 0.000 ) {
	  if ( $blue > $green ) {
		# blue - cyan
		$gray = $blue * ($low + $green * $delta / $blue);
	  }
	  else {
		# cyan - green
		$gray = $green * ($low + $delta + ($green - $blue)*$delta / $green);
	  }
	}
	else {
	  if ( $red > $green ) {
		# yellow - red
		$gray = $red * ( $high - $green * $delta / $red)
	  }
	  else {
		# green - yellow
		$gray = $green * ($high - $delta - ($green - $red)*$delta / $green); 
	  }
	}
  }
  else {
	$gray = $sum/3.0;
  }
}
#=======================================================================

#=======================================================================
#  subroutine unknown flag
#=======================================================================
sub unknownFlag {
  print "\n\t". $a . " is an unknown flag.\n";
  &printHelp;
}
#=======================================================================

#=======================================================================
#  subroutine print help message
#=======================================================================
sub printHelp {
  print "\npscol v$version: Patrick Joeckel (joeckel\@mpch-mainz.mpg.de)\n";
  print "Usage:\n";
  print "\t" . $0 . " [flags] <infilename> <outfilename>\n";
  print "\tAllowed flags are:\n";
  print "\t\t-h    \tprint this message and exit.\n";
  print "\t\t-gray \tconvert RGB colorscale to grayscale.\n";
  print "\t\t-0gray\tconvert RGB colorscale to grayscale (simple).\n";
  print "\t\t-cmyk \tconvert RGB to CMYK.\n";
  print "\tNote: Only for AFPL Ghostscript output (eps2eps, ps2ps) !!!\n\n";
}
#=======================================================================

